Compliance Change Tracking in Business Process Services

Regulatory compliance is an organization's adherence to laws, regulations, guidelines and specifications relevant to its business. Compliance officers responsible for maintaining adherence constantly struggle to keep up with the large amount of changes in regulatory requirements. Keeping up with the changes entail two main tasks: fetching the regulatory announcements that actually contain changes of interest, and incorporating those changes in the business process. In this paper we focus on the first task, and present a Compliance Change Tracking System, that gathers regulatory announcements from government sites, news sites, email subscriptions; classifies their importance i.e Actionability through a hierarchical classifier, and business process applicability through a multi-class classifier. For these classifiers, we experiment with several approaches such as vanilla classification methods (e.g. Naive Bayes, logistic regression etc.), hierarchical classification methods, rule based approach, hybrid approach with various preprocessing and feature selection methods; and show that despite the richness of other models, a simple hierarchical classification with bag-of-words features works the best for Actionability classifier and multi-class logistic regression works the best for Applicability classifier. The system has been deployed in global delivery centers, and has received positive feedback from payroll compliance officers.

==> challenges.tex <==
\section{Challenges}
\label{sec:challenges}
We discovered lot of interesting challenges both from software engineering and research perspective while working on this problem.

Problem 1 : Increasing list of news sources. With interactions from multiple Subject Matter Experts ()SME's) our applications could track large number of relevant sources for each identified regions. But we continue to discover new sources atleast for North America frequently. Therefore, there is a challenge and scope to expand our static list of sources through self learning.

Problem 2 : Certain times, updates are made to the already published article with no meta-data changes like created date/last update date.

Problem 3 : Most articles run more than 2 pages and language tend to be complex with no common pattern. Therefore compliance officers find it time consuming to read the entire article. Therefore there is a need for constraint(effective date, key change) based document summarization.


